The Power of Media Agencies in Ad Auctions: Improving Utility through Coordinated Bidding

The increasing competition in digital advertising induced a proliferation of media agencies playing the role of intermediaries between advertisers and platforms selling ad slots. When a group of competing advertisers is managed by a common agency, many forms of collusion, such as bid rigging, can be implemented by coordinating bidding strategies, dramatically increasing advertisers' value. We study the problem of finding bids and monetary transfers maximizing the utility of a group of colluders, under GSP and VCG mechanisms. First, we introduce an abstract bid optimization problem -- called weighted utility problem (WUP) -- , which is useful in proving our results. We show that the utilities of bidding strategies are related to the length of paths in a directed acyclic weighted graph, whose structure and weights depend on the mechanism under study. This allows us to solve WUP in polynomial time by finding a shortest path of the graph. Next, we switch to our original problem, focusing on two settings that differ for the incentives they allow for. Incentive constraints ensure that colluders do not leave the agency, and they can be enforced by implementing monetary transfers between the agency and the advertisers. In particular, we study the arbitrary transfers setting, where any kind of monetary transfer to and from the advertisers is allowed, and the more realistic limited liability setting, in which no advertiser can be paid by the agency. In the former, we cast the problem as a WUP instance and solve it by our graph-based algorithm, while, in the latter, we formulate it as a linear program with exponentially-many variables efficiently solvable by applying the ellipsoid algorithm to its dual. This requires to solve a suitable separation problem in polynomial time, which can be done by reducing it to a WUP instance.

==> paper Arxiv 1/contents/abstract.tex <==
The increasing competition in digital advertising induced a proliferation of \emph{media agencies} playing the role of intermediaries between \emph{advertisers} and \emph{platforms} selling ad slots. 
 %
 When a group of competing advertisers is managed by a common agency, many forms of collusion, such as bid rigging, can be implemented by coordinating bidding strategies, dramatically increasing advertisers' value.
 %
 We study the problem of finding \emph{bids} and \emph{monetary transfers} maximizing the utility of a group of colluders, under GSP and VCG mechanisms.
 %
 First, we introduce an abstract bid optimization problem---called \emph{weighted utility problem} (WUP)---, which is useful in proving our results.
 %
 We show that the utilities of bidding strategies are related to the length of paths in a directed acyclic weighted graph, whose structure and weights depend on the mechanism under study.
 %
 This allows us to solve WUP
 %\sout{the weighted utility problem} 
 in polynomial time by finding a shortest path of the graph.
 %
 Next, we switch to our original problem, focusing on two settings that differ for the \emph{incentives} they allow for.
 %
 Incentive constraints ensure that colluders do \emph{not} leave the agency, and they can be enforced by implementing monetary transfers between the agency and the advertisers.
 % under coordinated bidding.
 %
 In particular, we study the \emph{arbitrary transfers} setting, where any kind of monetary transfer to and from the advertisers is allowed, and the more realistic \emph{limited liability} setting, in which no advertiser can be paid by the agency.
 %
 In the former,
% \sout{setting}
 we cast the problem as  
 %\sout{a weighted utility problem} 
 a WUP instance and solve it by our graph-based algorithm, while, in the latter,
% \sout{setting}
 we formulate it as a 
 %\sout{LP} 
 linear program with exponentially-many variables 
% \sout{that is solved}
 efficiently solvable by applying the ellipsoid algorithm to its dual.
 %
 This requires to solve a suitable separation problem in polynomial time, which can be done by reducing it to 
 %\sout{the weighted utility problem}
 a WUP instance.

==> paper Arxiv 1/contents/introduction.tex <==
\section{Introduction}


Over the last years, digital advertising has been one of the main drivers of the growth of world market.
%
Remarkably, the vast majority of the companies employ digital tools to advertise their products or services, and the worldwide annual spent in digital advertising reached about 150 billion USD in 2020~\cite{iab2020iab}. 
%
Furthermore, most of the economic reports forecast that \emph{artificial intelligence} (AI) will fuel an increase of market value by almost 100\% over the next decade~\cite{McKinsey2018}. 
%
Indeed, AI tools have become widespread throughout digital advertising, enabling new opportunities that were not available before. Notable examples are in, \emph{e.g.}, auction design~\cite{Bachrach2014Optimising}, budget allocation~\cite{Nuara2018Combinatorial}, bidding opimization~\cite{He2013Game}, and multi-channel advertising~\cite{Nuara2019Dealing}.


Recent years have witnessed a proliferation of \emph{media agencies}, which claim to play the role of intermediaries between \emph{advertisers} and \emph{platforms} selling ad slots.
%
This has been driven by the increasing complexity of digital advertising---due to, \emph{e.g.}, a huge amount of available data and of parameters to be set on advertising platforms---and the rising competition among a growing number of advertisers.
%
% induced a proliferation of \emph{media agencies} that play the role of intermediaries between \emph{advertisers} and \emph{platforms} selling ad slots.
%
When a group of competing advertisers is managed by a common agency, it frequently happens that the agency has to place bids on behalf of different advertisers participating in the same ad auction.
%
This dramatically changes the strategic interaction underlying ad auctions, since agencies can coordinate advertisers' bidding strategies by implementing many forms of collusion---such as, \emph{e.g.}, bid rigging--, and, thus, they can increase advertisers' value.
%
% Since the number of agencies is orders of magnitude lower than the number of advertisers, it is more and more frequent that the same agency bids in the same auction on behalf of different, competing advertisers. This option dramatically changes the strategic interaction, as an agency can decrease its customers' payments by coordinating the bids.
%
In particular, simple examples show that colluding in ad auctions can reward the colluders with a utility that is arbitrarily larger than what they would get without doing that.
%
Moreover, a recent empirical study on real-world data by one of the major US agencies (Aegis-Dentsu-Merkle) shows that collusion is pervasive and leads to a significant reduction in the average cost-per-click \cite{RePEc:net:wpaper:1708}.


\paragraph{Original Contributions.}
%
We study the computational problem faced by a media agency that has to coordinate the bidding strategies of a group of colluders, under GSP and VCG mechanisms (details on the adoption of such mechanisms in ad auctions are provided in~\cite{10.1257/aer.104.5.442}).
%
We assume that the media agency knows the private valuations of the colluders (\emph{i.e.}, how much they value a click on their ad), and that it decides colluders' bids on their behalf. 
%
Moreover, the media agency is in charge of paying the auction mechanism for a click on an allocated ad, and at the same time it requires \emph{monetary transfers} to and from the colluders.
%
These are necessary to enforce some \emph{incentive constraints} ensuring that the colluders do \emph{not} leave the agency and participate in the ad auction individually. 
%
In this paper, we study two settings that differ on the kind of monetary transfers that they allow for: the \emph{arbitrary transfers} setting, where any kind of monetary transfer to and from the advertisers is allowed, and the more realistic \emph{limited liability} setting, in which no advertiser can be paid by the media agency.
%
Finally, we assume that the bids of the advertisers external to the media agency are drawn according to some probability distribution. 
%
As a first result, we introduce an abstract bid optimization problem---called \emph{weighted utility problem} (WUP)---, which works for any finite set of possible bid values and is useful in proving our main results in the rest of the paper.
%
In order to solve such a problem, we first show that the utilities of bidding strategies are related to the length of paths in a directed acyclic weighted graph, whose structure and weights depend on the mechanism under study (either GSP or VCG mechanism).
%
This allows us to solve  
%\sout{the weighted utility problem }
WUP instances in polynomial time by finding a shortest path of the graph.
%
Next, we switch the attention to the original media agency problem, starting from the arbitrary transfers setting.
%
A major challenge is dealing with a potentially continuous set of possible bids.
%
%\sout{First, we }
Notably, we show that it is possible to reduce the attention to a finite set of bidding strategies, only incurring in a small additive loss in the value of the obtained solution and relaxing the incentive constraints by a small additive amount.
%
The set is built by recursively splitting the interval of possible bid values, until one gets sub-intervals such that the probability that an external bid is in a given sub-interval is sufficiently small. 
%
Then, the resulting sub-intervals are used to define the desired finite set of bids.
%
In conclusion, we cast the problem as a
%\sout{weighted utility problem}
WUP instance
and solve it by our graph-based algorithm in polynomial time.
%
This gives a bi-criteria FPTAS for the original problem, since the approximation is in terms of both objective value and incentive constraints.
%
Finally, we study the limited liability setting.
%
In this case, we leverage the same finite set of bidding strategies defined for the arbitrary transfers setting in order to formulate the problem as a \emph{linear program} (LP) with exponentially-many variables and polynomially-many constraints.
%
Since we use only a finite set of bids, we need to relax the incentive constraints by an arbitrary small amount to guarantee the existence of a feasible solution.
%
%\sout{This can be solved} 
We solve the LP in polynomial time by applying the ellipsoid algorithm~\cite{grotschel1981ellipsoid} to its dual, which features polynomially-many variables and exponentially-many constraints.
%
This requires solving a suitable separation problem in polynomial time, which can be done by reducing it to 
%\sout{the weighted utility problem}
WUP instance. As in the arbitrary transfer setting, the resulting algorithm is a bi-criteria FPTAS.





\paragraph{Related Works.}
%
While a longstanding literature investigates the role of mediators in ad auctions---see, \emph{e.g.}, the seminal works by \citeauthor{Vorobeychik2008}~[\citeyear{Vorobeychik2008}] and \citeauthor{Ashlagi2009MediatorsIP}~[\citeyear{Ashlagi2009MediatorsIP}]---, collusion is currently emerging as one of the central problems in advertising as the adoption of AI algorithms can concretely support an agency to find the best collusive behaviors~\cite{OECD}. 
%
Motivated by the recent study by \citeauthor{RePEc:net:wpaper:1708}~[\citeyear{RePEc:net:wpaper:1708}], some works provide theoretical contributions to assess how collusion can be conducted by an agency.
%
\citeauthor{RePEc:inm:ormnsc:v:66:y:2020:i:10:p:4433-4454}~[\citeyear{RePEc:inm:ormnsc:v:66:y:2020:i:10:p:4433-4454}] study a setting in which there is no monetary transfer between the agency and bidders and provide equilibrium conditions. 
%
They show that, in simple settings, GSP is more inefficient than VCG both in terms of efficiency and revenue. \citeauthor{lorenzon}~[\citeyear{lorenzon}] studies a setting with two slots and three bidders which are all controlled by an agency in a GSP auction. Furthermore, a monetary transfer is possible. The author shows collusive stable behaviors in which the redistribution is uniform over the three bidders.



==> paper Arxiv 1/contents/limited_liability.tex <==
\section{Transfers with Limited Liability Setting}

\begin{comment}
Now we write the optimization problem (\ref{obj})-(\ref{c_limited}) when the colluders' bidding strategy $b^c$ is randomized. Variable $b^c$ is drawn from distribution $\Gamma^c$ with probability $\gamma_{b^c}$. We denote by $\gamma_{b}$ the probability of a bid vector $b \sim \Gamma$ composed of stochastic bid vectors from the colluders $b^c \sim \Gamma^c$ and the external agents $b^e \sim \Gamma^e$.
\begin{align} 
	\max_{q_i \geq 0, \gamma_{b^c} \geq 0} &\sum_{b} \gamma_b \sum_{i \in N} \mleft( \tilde{r}_i(b) - \tilde{\pi}_i(b) \mright) \label{obj_lim} \\
	\textnormal{s.t.} &\sum_{b} \gamma_b r_i(b) - q_i \geq t_i  \quad \forall i \in N \label{c_inc}\\
	&\sum_{i \in N} q_i \geq \sum_{b} \gamma_b \sum_{i} \pi_i(b) \label{c_transf}\\
	&\sum_{b^c} \gamma_{b^c} = 1 \label{c_prob}
\end{align}

\end{comment}

In this section, we provide an approximate solution to the media agency problem with limited liability constraints.
%
In particular, similarly to the arbitrary transfers setting, we design a bi-criteria FPTAS that returns solutions providing an arbitrary small loss $\varepsilon > 0$ with respect to the optimal value of the problem, by relaxing the IC constraints by $\varepsilon$.

As a first step, we show that we can restrict Problem~\eqref{lp:problem1} with LL constraints to work with the set $B^{c,p}$ by only incurring in a small loss in the objective function value and IC constraints satisfaction.
%
Notice that, Problem~\eqref{lp:problem1} with LL constraints restricted to discretized bids $B^{c,p}$ does not only have a smaller optimal value than Problem~\eqref{lp:problem1} with LL constraints, but it can also result in an infeasible problem, since Assumption~\ref{as_unica} is \emph{not} necessarily satisfied for a discretized bidding strategy $b^c \in B^{c,p}$.
%
However, we can prove that, given a probability $p \in [0,1]$, the following LP~\eqref{lp:Limit} that uses only bids in $B^{c,p}$ and relaxes the IC constraints of quantity $p$ is feasible and has value at least $OPT-pn_c$, where $OPT$ is the optimal value of Problem~\eqref{lp:problem1} with LL constraints.
%
\begin{subequations}\label{lp:Limit}
\begin{align} 
\max_{q \geq 0, \gamma \in \Delta_{B^{c,p}}} &\sum_{b^c \in B^{c,p}} \gamma_{b^c} \sum_{i \in N_c}  \tilde{r}_i(b^c) - \tilde{\pi}_i(b^c)  \label{obj_lim2} \quad  \textnormal{s.t.}\\
 &\hspace{-1cm}\sum_{b^c \in B^{c,p}} \gamma_{b^c} \tilde r_i(b^c) - q_i \geq t_i -p  \qquad \forall i \in N_c \label{c_inc2}\\
 &\hspace{-1cm}\sum_{i \in N_c} q_i \geq \sum_{b^c \in B^{c,p}} \gamma_{b^c} \sum_{i \in N_c} \tilde \pi_i(b^c). \label{c_transf2}
\end{align}
\end{subequations}

Formally, we prove the following:
%
\begin{restatable}{lemma}{Feasible} \label{lm:feasible}
	LP~\eqref{lp:Limit} is feasible.
	%
	Moreover, the optimal value of LP~\eqref{lp:Limit} is at least $OPT-pn_c$, where $OPT$ is the optimal value of Problem~\eqref{lp:problem1} with LL constraints.
\end{restatable}


In the rest of the section, we will provide an algorithm to solve LP~\eqref{lp:Limit} by using the ellipsoid method.
%
In order to do that, we use the dual LP~\eqref{lp:dual}, in which variables $y=\{y_1, \ldots,y_{n_c}\}$, $x$, and $z$ are related to Constraints~\eqref{c_inc2},~\eqref{c_transf2}, and the constraint $\gamma \in \Delta_{B^{c,p}}$, respectively.
\begin{subequations} \label{lp:dual}
\begin{align} 
	\min_{y \leq 0,x,z} & \,\, \sum_{i \in N_c} (t_i-p) y_i + z  \quad \textnormal{s.t.} \label{obj_lim_dual} \\
	 &\sum_{i \in N_c} y_i \tilde r_i(b^c) - x \sum_{i \in N_c} \tilde \pi_i(b^c) + z \geq \nonumber \\
	& \qquad  \sum_{i \in N_c} \tilde r_i(b^c)-\tilde \pi_i(b^c) \quad\quad\quad   \forall b^c \in B^{c,p} \label{dual:2}\\
	&-y_i +x \geq 0   \hspace{3cm}\forall i \in N_c. \label{dual:3}
\end{align}
\end{subequations}

By Lemma~\ref{lm:feasible}, the primal LP~\eqref{lp:Limit} is feasible (and bounded), and, thus, it holds strong duality.
%
As a consequence, in order to provide a polynomial-time algorithm to solve LP~\eqref{lp:Limit}, it is enough to apply the ellipsoid method to the dual LP~\eqref{lp:dual}, which can be done in polynomial time since the latter has polynomial-many variables and exponentially-many constraints.
%
This is possible by providing a polynomial-time separation oracle that, given an assignment of values to the variables as input, returns a violated constraint (if any).
%
Since there are only polynomially-many Constraints~\eqref{dual:3}, we can check if one of them is violated in polynomial time.
%
Moreover, in order to find whether there exists a violated Constraint~\eqref{dual:2}, it is sufficient to solve the weighted utility problem in Equation~\eqref{obj_wup} by setting $\hat{y_i} =(1-y_i)$ for each $i \in N_c$ and $\hat x=x-1$.
%
By Theorem~\ref{th_poly}, this can be done in polynomial time with computing a shortest path of a suitable graph.
%
Hence, we can prove the following theorem.
%
\begin{restatable}{theorem}{ExistPloyAlgorithm}
		Given $\epsilon>0$, there exists an algorithm that runs in time polynomial in the instance size and $\frac{1}{\varepsilon}$ and returns an $\varepsilon$-IC and IR solution to Problem~\eqref{lp:problem1} with LL constraints having value at least $OPT-\varepsilon$, where $OPT$ is the optimal value of Problem~\eqref{lp:problem1} with LL constraints.
\end{restatable}






==> paper Arxiv 1/contents/preliminaries.tex <==
\section{Preliminaries}

We study the problem of coordinated bidding faced by a media agency in ad auctions, with both GSP and VCG payments.
%
In this setting, there is a set $N_c \coloneqq \{1,\ldots,n_c\}$ of \emph{advertisers} (or \emph{agents}), whose advertising campaigns are managed by a common media agency. 
%
Moreover, there is another set $N_e \coloneqq \{1,\ldots,n_e\}$ of advertisers who are \emph{not} part of the agency, but participate to the ad auction individually.
%
In this work, we refer to the former as \emph{colluders}, while we call the latter \emph{external agents}.
%
For the ease of presentation, we let $N \coloneqq N_c \cup N_e$, and, with a slight abuse of notation, we sometimes write $N \coloneqq \{1,\ldots,n\}$ by renaming the agents, where $n=n_c+n_e$.
%
The advertisers compete for displaying their ads on a set $M \coloneqq \{1,...,m\}$ of \emph{slots}, with $m \leq n$.
%
Each agent $i \in N$ has a \emph{private valuation} $v_i \in [0,1]$ for an advertising slot, which reflects how much they value a click on their ad.
%
Moreover, each slot $j \in M$ is associated with a \emph{click through rate} parameter $\lambda_j \in[0,1]$, encoding the probability with which the slot is clicked by a user.\footnote{For the ease of presentation, we assume that the click through rate only depends on the slot and \emph{not} on the ad being displayed. This dependence can be easily captured by interpreting $v_i$ as an expected value w.r.t.~clicks once the user observed the slot.
%\sout{All the results in this paper can be generalized to the case in which the click through rate also depends on the ad.}
} 
%
Each agent $i \in N$ participates in the ad auction with a \emph{bid} $b_i \in [0,1]$, representing how much they are willing to pay for a click on their ad.
%
We denote by $b = (b_1, \ldots , b_{n})$ the bid profile made by all the agents' bids.
%
We also let $b^c = (b^c_1, \ldots , b^c_{n_c})$ be the profile of colluders' bids (also called \emph{bidding strategy}), while $b^e = (b^e_1, \ldots , b^e_{n_e})$ is the profile of external agents' bids.
%
For the ease of notation, we sometimes write $b = (b^c,b^e)$ to denote the profile made by all the bids in $b^c$ and $b^e$.
%
Finally, the media agency knows the valuations $v_i$ of all the colluders $i \in N_c$, and it decides the bid profile $b_i^c$ on their behalf.
%
Additionally, the media agency defines a monetary \emph{transfer} $q_i \in [-1,1]$ for each colluder $i \in N_c$.
%
We adopt the convention that, if $q_i > 0$, then the transfer is from the agent to the agency, while, if $q_i < 0$, then it is the other way around.\footnote{Notice that there are some scenarios in which it is in the interest of the media agency to pay a colluder in order to ensure that they stay in the agency; see Example~\ref{ex_agencycoord_at} in the Supplementary Material.}

In this work, we assume w.l.o.g. that the bids in a profile $b = (b_1, \ldots , b_{n})$ are ordered by decreasing value of $b_i$, and that the same holds for $b^c$ and $b^e$.
%
Moreover, w.l.o.g., we assume that the sots are ordered so that $\lambda_1 \geq \ldots \geq \lambda_m$.




The auction goes on as follows.
%
First, the media agency selects a bidding strategy $b^c = (b^c_1, \ldots , b^c_{n_c})$ and requires a transfer $q_i$ from each colluder $i \in N_c$. 
%
Then, external agents individually report their bids to the auction mechanism, resulting in a profile $b^e = (b^e_1, \ldots , b^e_{n_e})$, while the media agency reports bids $b^c$ on behalf of the colluders.
%
Finally, given all the agents' bids $b = (b^c,b^e)$, the mechanism allocates an ad to each slot and defines an \emph{expected payment} $\pi_i(b) \in [0,1]$ for each agent $i \in N$, where the expectation is with respect to the clicks.
%
The media agency is responsible of paying the mechanism on behalf of the colluders.
%
%, and, finally, pays the sum of payments $p_i$, for $i \in N^c$, to the mechanism.
%
%We define an allocation function $f$ s.t. $f_i(b)=j$ if ad $i \in A$ is assigned to slot $j \in M$, given a bid profile $b$, and $f_i(b) = \bot$ if ad $i$ is not displayed. 
%We also define a set of allocations $K$. We denote by $k(b) \in K$ an allocation, given a bid profile $b$, such that $k(b) \coloneqq \{(i,j) \in A \times (M \cup \{\bot\}) : f_i(b)=j || \not\exists i' : f_{i'}(b)=f_i(b)=j, \forall j \in M \}$.


% Given a payment vector $p = \{p_1, \ldots, p_n\}$, 
%
Given a bid profile $b = (b_1, \ldots , b_{n})$ and assuming w.l.o.g. that each bidder $i \in [m]$ is assigned to slot $i$, we denote bidder $i$'s \emph{expected revenue} as $r_i(b) \coloneqq \lambda_{i} v_i$, while bidder $i$'s \emph{expected utility} is $u_i(b) \coloneqq r_i(b) - q_i$.\footnote{We denote with $[m]$ the set $\{1, \ldots, m\}$.}
%
% the expected utility of agent $i$ and by $\pi_i(b) = \lambda_{j} p_i$ the expected payments related to agent $i$ that the agency pays to the mechanism.
%
Instead, the expected utility of the agency is $\sum_{i \in N_c} (q_i - \pi_i(b))$.
%
We also denote with $U $ the cumulative expected utility of all the colluders and the media agency.
%
Formally, $U \coloneqq \sum_{i \in N_c} (r_i(b) - \pi_i(b) )$.


Next, we review GSP and VCG mechanisms in ad auctions (see the book by~\citeauthor{nisan2001algorithmic}~[\citeyear{nisan2001algorithmic}] for their general description).
%
Given a bid profile $b = (b_1, \ldots, b_n)$, both mechanisms orderly assign the first $m$ agents, who are those with the highest bids, to the first $m$ slots, which are those with the highest click through rates.
%
Moreover, the mechanisms assign the following expected payments.
%
\begin{itemize}
	\item \emph{GSP mechanism}: $\pi_i^{\GSP}(b) \coloneqq \lambda_i b_{i+1}$ for each agent $i \in [m]$, and $\pi_i^{\GSP}(b) = 0$ for all the other agents.
	%
	\item \emph{VCG mechanism}: $\pi_i^{\VCG}(b) \coloneqq \sum_{j=i+1}^{m+1} b_{j}(\lambda_{j-1} -\lambda_{j} )$ for each agent $i \in [m]$, where we let $\lambda_{m+1} = 0$, and $\pi_i^{\VCG}(b) = 0$ for all the other agents.
\end{itemize}

The VCG payments are such that each agent is charged a payment that is equal to the externalities that they impose on other agents.
%
This makes the VCG mechanism \emph{truthful}, which means that it is a dominant strategy for each agent to report their true valuation to the mechanism, namely $b_i =   v_i$ for every $i \in N$. 
%
This is \emph{not} the case for the GSP mechanism.



%In truthful mechanisms, such as standard VCG auction, allocation and payments are defined so that it is a dominant strategy for each agent to report their true valuation to the mechanism, namely $b_i =   v_i$ for every $i \in N$. 
%%
%Consider a set of agents $N$ and their bids $b$.
%%
%The allocation implemented by both the GSP and the VCG mechanism orderly assigns the first $m$ agents (those with the highest bids) to the first $m$ slots (those with the highest click through rates).
%%
%At the same time, assuming w.l.o.g. that bidder $i$ is assigned to slot $i$, the mechanisms assign the following expected payment.
%
%\paragraph{GSP Payment Rule.}
%GSP expected payment is $\pi_i^{\GSP}(b) \coloneqq \lambda_i b_{i+1}$ to each agent $i \in \{1, \ldots, m\}$. 
%%
%%The corresponding expected utility is $u_i^{\GSP}(b)= \lambda_{i}v_i - \pi_i^{\GSP}(b) =\lambda_{i}(v_i -b_{i+1})$.
%%, where, for the ease of notation, we let $\lambda_{m+1} = 0$.
%%
%The payment is zero for all the other agents.
%%
%%
%%We define agent $i$'s payment as $p_{i} = \max\{b_{i+1}, \max_{j : l_j < b_i}\{l_j\}\}$, \emph{i.e.}, the maximum between the bid $b_{i+1}$ of the next colluder and the highest threshold from $l$ that is smaller that $b_i$. If $n \leq m$, the $n$-th agent pays zero.
%%
%
%\paragraph{VCG Payment Rules.}
%VCG payment rule charges each agent their externality by setting expected payment $\pi_i^{\VCG}(b) \coloneqq \sum_{j=i+1}^{m+1} b_{j}(\lambda_{j-1} -\lambda_{j} )$ to each agent $i \in \{1, \ldots, m\}$, where, for the ease of notation, we let $\lambda_{m+1} = 0$. 
%%The corresponding expected utility of agent $i$ is $u_i^{\VCG}(b)= \lambda_i v_i - \pi_i^{\VCG}(b)$.
%%
%The payment is zero for all the other agents.
%%
%%\[\pi_i = \max_{k \in K_{-i}} \mleft\{ \sum_{h \in N \backslash \{i\}} \lambda_{f_k(h)} v_h \mright\} - \sum_{h \in N \backslash \{i\}} \lambda_{f(h)}v_h\]
%%where $K_{-i}$ is the set of allocations where bidder $i$ is not included (\emph{i.e.} $f(i)=\bot$).
%%
%
%
%%In the ads auction setting, agent $i$'s true type is the private value $v_i$, while the type reported to the auctioneer is the bid $b_i$. The auction mechanism is \emph{direct-revelation} when the agents reports their true types (\emph{i.e.}, $v=b$), otherwise it is called \emph{indirect-revelation}. 
%%
%%Now we review the VCG and the GSP mechanisms, which will be used throughot the paper.











==> paper Arxiv 1/contents/problem.tex <==
\section{Problem Formulation}

In this section, we introduce the optimization problem faced by the media agency.
%
In words, the goal of the media agency is to find a bidding strategy $b^c= (b^c_1, \ldots, b^c_{n_c})$ that coordinates colluders' bids in a way that maximizes the cumulative expected utility $U$, while at the same time guaranteeing that they are incentivized to be part of the media agency.
%
The rest of the section is devoted to formally defining such a problem.
%, together with some of its general properties that will be useful in the remaining of the paper.


Before introducing the optimization problem, let us notice that knowing the valuations of all the colluders allows the media agency to improve the cumulative expected utility $U$ with respect to the case in which all the bidders act individually.
%, by reducing external bidders' utilities.
%
% A media agency controls a set $N^c$ of agents and is able to jointly optimize their bidding strategies. The agency can rely on the information asymmetry in its favor due to the knowledge of the private vauations of $n^c$ agents participating in the same auction. On the other hand, each external agent only knows their own private valuation.
%
This is formalized by the following proposition, whose proof is Example~\ref{ex_agencycoord} in the Supplementary Material.
%
\begin{proposition}\label{prop_motivation}
	 The cumulative expected utility $U$ may be arbitrarily larger than the sum of the colluders' expected utilities when they participate in the ad auction individually.
\end{proposition}
%
% Proposition~\ref{prop_motivation} is proved by Example~\ref{ex_agencycoord} in the Appendix.



% We analyze from the agency perspective how to coordinate the group of colluders in order to maximize their expected cumulative utility $U$. 
%
%
In general, the media agency may adopt a \emph{randomized} bidding strategy in order to maximize $U$.
%
By letting $B^c$ be the set of all the possible colluders' bid profiles $b^c= (b^c_1, \ldots, b^c_{n_c})$, we denote by $\gamma \in \Gamma$ any randomized bidding strategy, where $\Gamma$ is the set of all the probability distributions over $B^c$.
%
% and we define $\Gamma$ as a set of probability distributions over the set of bid profiles $B^c$. We denote with $\gamma \in \Gamma$ a probability distribution over $B^c$.
%and with $b^c \sim \gamma^c$ a sample from the distribution $\gamma^c$. 
%
Moreover, whenever $\gamma \in \Gamma$ has a finite support, we denote with $\gamma_{b^c}$ the probability of choosing a bidding strategy $b^c \in B^c$.


In this work, unless stated otherwise, we consider the case in which the bid profile $b^e= (b^e_1, \ldots, b^e_{n_e})$ of the external agents is drawn from a probability distribution $\gamma^e$.
%
%, where $b^e \sim \gamma^e$ is a sample from the distribution $\gamma^e$.
%
Then, we define the expected revenue of bidder $i \in N_c$ for any bidding strategy $b^c \in B^c$ as $\tilde r_i(b^c) \coloneqq \mathbb{E}_{b^e \sim \gamma^e} r_i(b^c,b^e)$,
%, while the expected utility of bidder $i$ given a randomized bidding strategy $\gamma \in \Gamma$ is written as $\mathbb{E}_{b^c \sim \gamma} \tilde u_i(b^c)$.
% Then, we define the expected utility of bidder $i \in N$ for any bidding strategy $b^c \in B^c$ as $\tilde u_i(b^c) \coloneqq \mathbb{E}_{b^e \sim \gamma^e} u_i(b^c,b^e)$, while the expected utility of bidder $i$ given a randomized bidding strategy $\gamma \in \Gamma$ is written as $\mathbb{E}_{b^c \sim \gamma} \tilde u_i(b^c)$. \textcolor{red}{check se serve tenere la def di $\tilde{u}$}
%
while their expected payment is as $\tilde \pi_i(b^c) \coloneqq \mathbb{E}_{b^e \sim \gamma^e} \pi_i(b^c,b^e)$.
%
%  We denote by $\gamma_{b^e}$ the probability of $b^e$. 
%5\textcolor{red}{supponendo che sono discrete, è ok?}.
% 
%We denote by $\gamma$ the probability of vector $b=(b^c,b^e)$ which is the joint probability of drawing vectors $b^c$ and $b^e$.
%
In the rest of the paper, we assume that all algorithms have access to an oracle that returns the value of the expectations $\tilde r_i(b^c)$, and $\tilde \pi_i(b^c)$ for a bidding strategy $b^c\in B^c$ given as input.\footnote{Our results can be easily extended---only incurring in a small additive loss in cumulative expected utility---to the case in which the distribution $\gamma^e$ is unknown, but the algorithms have access to a black-box oracle that returns i.i.d.~samples drawn according to $\gamma^e$ (rather than returning expected values).}


% We study the problem in which the agency can use a randomized bidding strategy $\gamma$ and can require transfers $\{q_i\}_{i \in N^c}$ from the colluders.
%
The following Problem~\eqref{lp:problem1} encodes the maximization problem faced by the media agency, where the meaning of IC and IR constraints is described in the following.
%, where the IC and IR constraints are defined below.
%
\begin{subequations}\label{lp:problem1}
\begin{align}
 	\max_{q ,\gamma \in \Gamma} & \,\, \sum_{i \in N_c} \mathbb{E}_{b^c\sim \gamma}\mleft[\tilde r_i(b^c) - \tilde\pi_i(b^c)\mright] \quad \text{s.t.} \label{obj} \\
 	& \textnormal{IC}: \,\,\, \mathbb{E}_{b^c\sim \gamma}\mleft[\tilde r_i(b^c)\mright] - q_i \geq t_i  \hspace{1.3cm}  \forall i \in N_c  \label{c_incentive}\\
 	& \textnormal{IR}: \,\,\, \sum_{i \in N_c} q_i \geq \sum_{i \in N_c} \mathbb{E}_{b^c \sim \gamma}\mleft[\tilde \pi_i(b^c)\mright].    \label{c_transfer}
\end{align}
\end{subequations}
%
%where variable $q$ is useful to model constraints that we introduce below.


%The elements of Problem~\eqref{lp:problem1} are defined as follows:
%%
%\begin{itemize}
%\item Objective~\eqref{obj} encodes the cumulative expected utility $U$ of the colluders and the media agency, in expectation with respect to the randomized bidding strategy $\gamma$.
%%
%\item Constraints~\eqref{c_incentive}---called \emph{incentive compatibility} (IC) constraints---ensure that the colluders are incentivized to be part of the media agency, rather than leaving it and participating in the ad auction as external agents.
%%
%In particular, they guarantee that each colluder $i \in N_c$ achieves at least a minimum expected utility $t_i$, where the values $t_i \in [0,1]$ for $i \in N_c$ are given as input.\footnote{To the best of our knowledge, in the literature there is only one work by~\citeauthor{bachrach2010honor}~[\citeyear{bachrach2010honor}] that formalizes IC constraints for a setting that is similar to ours. \citeauthor{bachrach2010honor}~[\citeyear{bachrach2010honor}]~takes inspiration from the concept of core in cooperative game theory in order to define suitable IC constraints. However, this approach has many downsides. The most relevant issue of such an approach is that it is \emph{not} computationally viable, since computing the core would require exponential time in the number of colluders $n_c$.}
%%
%\item Constraint~\eqref{c_transfer} is an \emph{individual rationality} (IR) guarantee for the media agency.
%%
%Since the agency corresponds to the mechanism a payment $\sum_{i \in N_c} \mathbb{E}_{b^c \sim \gamma}[\tilde \pi_i(b^c)]$ in expectation over the clicks, the constraint requires that the sum of transfers $\sum_{i \in N_c} q_i$ covers the payment, so that the expected utility to the agency is positive.
%%
%\end{itemize}

\noindent The elements of Problem~\eqref{lp:problem1} are defined as follows.

Objective~\eqref{obj} encodes the cumulative expected utility $U$ of the colluders and the media agency, in expectation with respect to the randomized bidding strategy $\gamma$.
%

Constraints~\eqref{c_incentive}---called \emph{incentive compatibility} (IC) constraints---ensure that the colluders are incentivized to be part of the media agency, rather than leaving it and participating in the ad auction as external agents (notice that these constraints naturally enforce bidders' individual rationality).
%
In particular, they guarantee that each colluder $i \in N_c$ achieves at least a minimum expected utility $t_i$, where the values $t_i \in [0,1]$ for $i \in N_c$ are given as input.\footnote{To the best of our knowledge, in the literature there is only one work by~\citeauthor{bachrach2010honor}~[\citeyear{bachrach2010honor}] that formalizes IC constraints for a setting that is similar to ours. \citeauthor{bachrach2010honor}~[\citeyear{bachrach2010honor}]~takes inspiration from the concept of core~\cite{cooperativegames} in cooperative games in order to define suitable IC constraints. However, this approach has many downsides. The most relevant issue of such an approach is that it is \emph{not} computationally viable, since computing the core would require exponential time in the number of colluders $n_c$.}
%

Constraint~\eqref{c_transfer} is an \emph{individual rationality} (IR) guarantee for the media agency.
%
Since the agency corresponds to the mechanism a payment $\sum_{i \in N_c} \mathbb{E}_{b^c \sim \gamma}[\tilde \pi_i(b^c)]$ in expectation over the clicks, the constraint requires that the sum of transfers $\sum_{i \in N_c} q_i$ covers the payment, so that the expected utility to the agency is positive.
%




In the following, we sometimes relax IC constraints by using $\delta$-IC constraints, for $\delta > 0$, which are defined as follows:
%
\begin{align}\label{c_eps_incentive}
& \delta\textnormal{-IC}: \,\,\, \mathbb{E}_{b^c\sim \gamma} \mleft[\tilde r_i(b^c)\mright] - q_i \geq t_i -\delta & \forall i \in N_c.
\end{align}


% In general, it may be the case that $q_i<0$ for some $i \in N_c$, meaning that agent $i$ is paid by the media agency (see Example~\ref{ex_agencycoord_at}).
%
%$T_i < - E_{b \sim \gamma_b} \mleft[\pi_i(b)\mright]$, and the payments of other colluders are arbitrarily redistributed s.t. $E_{b \sim \gamma_b} \mleft[u_i(b)\mright] > E_{b \sim \gamma_b} \mleft[r_i(b)\mright]$ (see Example \ref{ex_agencycoord_at}).
%
In the following, we call the scenario described so far, in which transfers $q_i$ could be negative, the \emph{arbitrary transfers} setting.
% since, in general, it might be the case that the transfer associated with an agent is negative. 
%, the scenario modeled by the optimization problem (\ref{lp:problem1}).
%
%
Monetary transfers from the media agency to the agents are \emph{not} always feasible in practice. 
%
Indeed, in some real-world scenarios a media agency could potentially loose customers by adopting a strategy for which some agents pay and some others are paid for participating in the same auction.
%
% Moreover, in real-world scenarios, it is quite natural that an agency providing a service requires to be paid by its customers, and \emph{not} the other way around.
%
For these reasons, we introduce and study a second scenario, which we call \emph{transfers with limited liability} setting, where no agent is paid by the agency.
%\footnote{Notice that, from a theoretical point of view, there may be problem instances for which it could be worthwhile to pay advertisers for staying under the agency. From the agency perspective, this is equivalent to pay for acquiring knowledge of those agents' private valuations and for leaving them out of the auction by setting their bid equal to zero, which could be crucial to enlarge the cumulative utility $U$. This motives the study of the arbitrary transfer setting.
%\textcolor{red}{NOTA RISCHIOSA. FORSE STIAMO SMINUENDO TROPPO IL CASO ARBITRARY TRANSFERS.}}
%
% Therefore, the term \emph{limited liability} refers to the agency which is willing to redistribute payments under certain restrictions.
%
In such setting, Problem~\eqref{lp:problem1} is augmented with the following additional \emph{limited liability} (LL) constraints on the monetary transfers $q_i$:
\begin{align}
	& \textnormal{LL}: \,\,\, q_i \geq 0  & \forall i \in N_c.   \label{c_limited}
\end{align}
%
As we show in Section~\ref{sec:arbitrary}, there always exists an optimal solution to Problem~\eqref{lp:problem1} without LL constraints that is \emph{not} randomized.
%
The same does not hold for the problem with LL constraints, in which an optimal bidding strategy may be randomized, as in Example~\ref{ex_randombest} in the Supplementary Material.



%
We conclude by introducing the following assumption on the values $t_i$, guaranteeing that Problem~\eqref{lp:problem1} is feasible.\footnote{The proofs of all the results are in the Supplementary Material.}
%
%As it easy to see, problem \ref{lp:problem1} is unfeasible when the parameters $t_i$ are too large.
% In particular, our assumption reads as follows.
%
\begin{assumption} \label{as_unica}
	There always exists a bidding strategy $b^c \in B^c$ such that $\tilde r_i(b^c) - \tilde \pi_i(b^c) \ge t_i $ for all $i \in N_c$.
	%
	%The minimum guaranteed utilities $\{t_i\}_{i \in N^c}$ are such that there exists a bid profile $b^c \in B^c$ such that: 
	%\[\tilde u_i(b^c)\ge t_i \ \ \forall i \in N^c .\]
\end{assumption}
%
%
% Notice that even if Assumption \ref{as_unica} can be replaced with less stringent assumptions, \emph{e.g.}, in the arbitrary transfers setting it can be replaced by $\sum_{i \in N^c}\tilde u_i(b^c)\ge \sum_{i \in N^c} t_i$, we show that it is reasonable in practice.
%
\begin{restatable}{proposition}{PropNonRand}
	When Assumption \ref{as_unica} holds, there always exists a non-randomized feasible solution to the Problem~\eqref{lp:problem1} with LL constraints.
\end{restatable}
%
In Appendix~\ref{appendixA} of the Supplementary Material, we provide some examples of natural choices for the values $t_i$, which arise from allocation and payment rules of the considered auction mechanisms and satisfy Assumption~\ref{as_unica}.
%
%These examples suggest that there exists a na\"ive bidding strategy for the colluders that is reasonable for the problem under study and that the values $t_i$ can be set so that at least such a bidding strategy is feasible for Problem~\eqref{lp:problem1} with LL constraints.

%\begin{example}\label{ex_tGSP}
%	Consider GSP mechanism and a reasonable fixed strategy for the colluders, fixed with rres
%	
%	Consider the optimization problem (\ref{obj})-(\ref{c_limited}) and a GSP auction mechanism. \textcolor{red}{bidding strategy che porta a equil VCG (max SW)}
%	
%	\textcolor{red}{PROBLEMA: bidding strat è Balanced Bidding di Cary2007GreedyStrat e porta a utilities VCG, ma dovrei poter assicurare che anche external bids seguano questa strategia}
%\end{example}

%\textcolor{red}{
%	\begin{proposition}
%		When Assumption \ref{as_unica} holds, there exist a deterministic feasible solution to the optimization problem \eqref{lp:problem1}, with LL constraint.
%	\end{proposition}
%	%
%	\begin{proof}
%		It can be show
%	\end{proof}
%	%
%	For instance, in Example \ref{ex_randombest}, Assumption \ref{as_unica} is satisfied and there exist a non-randomized bid profile $b^c$ which is a feasible solution to the optimization problem \eqref{lp:problem1} with LL.
%	%
%	Notice that, there exist some problem instances for which Assumption \ref{as_unica} is not satisfied, and all the feasible solutions to problem \eqref{lp:problem1} with LL are randomized bidding strategies, as in Example \ref{ex_agencycoord_ll}.
%}



\begin{comment}


Moreover, Example \ref{ex_agencycoord_ll} shows how the choice of parameter $t$ determines the existence of a feasibile solution for the optimization problem. In the next sections we need the following conditions.
\begin{assumption} \label{as_ar}
	There exist a feasible solution to the optimization problem (\ref{obj})-(\ref{c_transfer}) if \textcolor{red}{or iff} 
	\begin{align}
		\sum_{i \in N^c} t_i \leq \max_{\gamma_{b^c}} \sum_{i \in N^c} E_{b \in \gamma_b} \mleft[u_i(b) \mright].
	\end{align}
\end{assumption}

\begin{assumption} \label{as_ll}
	There exist a feasible solution to the optimization problem (\ref{obj})-(\ref{c_limited}) if \textcolor{red}{or iff} 
	\begin{align}
		t_i \leq \max_{\gamma_{b^c}} E_{b \in \gamma_b} \mleft[u_i(b)\mright].
	\end{align}
\end{assumption}

Notice that when Assumption~\ref{as_ll} holds, also Assumption~\ref{as_ar} is satisfied.
%

\end{comment}






%The optimization problem is the following.

%\begin{subequations}
%\begin{align}
%	&\max_{b \in B} & \sum_{i=1}^N u_i \label{obj_fun} \\
%	&\text{s.t.} & \sum_{i=1}^N u_i \geq \sum_{i=1}^N t_i , \label{incentive}
%\end{align}
%\end{subequations}

==> paper Arxiv 1/contents/transferrable.tex <==
\section{Weighted Utility Problem}\label{sec:weighted}

In this section, we provide a polynomial-time algorithm for an abstract bid optimization problem 
%\sout{, which we call \emph{weighted utility problem}.}
we call \emph{weighted utility problem} (WUP).
%, showing that it admits a polynomial-time algorithm. 
%
This will be crucial in the following sections in order to solve Problem~\eqref{lp:problem1} with or without LL constraints.


Let $\mathcal{B}^c \coloneqq \{\bar{b}^c_1, \ldots, \bar{b}^c_d\}$ be a discrete set of $d$ different bid values, with $\bar{b}^c_1 \geq \ldots \geq \bar{b}^c_d$.
%
Moreover, given a bidding strategy $b^c \in B^c$ such that $b^c_i \in \mathcal{B}^c$ for all $ i \in N_c$, we write $b^c \in \bar{B}^c$ to express that each element of $b^c$ belongs to $\mathcal{B}^c$.
%

Then, WUP
%\sout{the weighted utility problem}
reads as follows:
%
\begin{align} \label{obj_wup}
	\max_{b^c \in \bar{B}^{c}} \sum_{i \in N_c}\mleft( \hat{y}_i \, \tilde{r}_i(b^c) - \hat{x} \, \tilde{\pi}_i(b^c)\mright),
\end{align}
where $\hat{y}_i \ge 0$ for all $ i \in N_c$ and $\hat{x}\ge 0$.
%
A solution to Problem~\eqref{obj_wup} is a bidding strategy $b^c \in \bar{B}^c$ that maximizes the sum of suitable \emph{weighted} utilities of the colluders, which are defined so that colluder $i$'s expected revenue $\tilde{r}_i(b)$ is weighted by coefficient $\hat{y}_i$, while their expected payment $\tilde{\pi}_i(b)$ is weighted by coefficient $\hat{x}$.
%
In the following, for the ease of notation, for any $b^c \in \bar{B}^c$, we let $u_i^{\w}(b^c) \coloneqq \hat{y}_i \, \tilde{r}_i(b^c) - \hat{x} \, \tilde{\pi}_i(b^c)$ for every $i \in N_c$.
%
Notice that, when $\hat{y}_i=1$ for all $ i \in N_c$ and $\hat{x}=1$, then the objective of Problem~\eqref{obj_wup} coincides with the cumulative expected utility $U$.
%

\begin{figure}[!htp]
	\centering
	\includegraphics[scale=0.7]{img/graphcropped.pdf}
	\caption{Structure of the graph when $N_c=\{1,2,3\}$ and $b^c_i \in \mathcal{B}^c=\{\bar{b}^c_1, \bar{b}^c_2, \bar{b}^c_3\}$ for all $ i \in N_c$.} 
	\label{fig:graph}
\end{figure}

As a first step, we consider Problem~\eqref{obj_wup} in which the profile of external agents' bids $b^e$ is fixed, which reads as follows: 
%
\begin{align} \label{obj_wup_fix}
	\max_{b^c \in \bar{B}^{c}} \sum_{i \in N_c} \mleft(\hat{y}_i \, r_i(b^c,b^e) - \hat{x} \, \pi_i(b^c, b^e)\mright).
\end{align}
% where $\hat{y}_i > 0$, $\forall i \in N^c$ and $\hat{x}> 0$.
%
For the sake of presentation, we first provide our results for Problem~\eqref{obj_wup_fix}, and, then, we show how they can be extended to Problem~\eqref{obj_wup}, where the bids of external agents are stochastic.



The main idea underpinning our results is to map Problem~\eqref{obj_wup} into a \emph{shortest path problem} \cite{10.1007/BF01386390}.  
%
Specifically, we show that the weighted utilities of bidding strategies are related to the length of paths in a particular directed acyclic weighted graph, whose structure and weights derive from the considered auction mechanism.
%
The following lemma is crucial for the construction of the graph.
%~\footnote{The proofs of all the results can be found in the Appendix.}
%
\begin{restatable}{lemma}{OrderedBidding} \label{lem_bidorder}
	If the colluders in $N_c$ are ordered so that $\hat{y}_1 v_1 \geq \ldots \geq \hat{y}_{n_c} v_{n_c}$, then, for every $b^e$, any optimal bidding strategy $b^{c*} \in \bar{B}^c$ for Problem~\eqref{obj_wup_fix} is such that $b_1^{c*} \geq \ldots \geq b_{n_c}^{c*}$.
	%
	% Given a set of colluders $N^c$ ordered in decreasing value of weighted valuations $\hat{y}_1 v^c_1 \geq \ldots \geq \hat{y}_n v^c_{n}$, the optimal bidding strategy $b^{c*}$ for the optimization problem (\ref{obj_wup}) is such that $b_1^{c*} \geq \ldots \geq b_n^{c*}$, $\forall b^e$.
\end{restatable}
%
%\noindent We build the graph as follows.

%The set of vertices $V$ contains $d n_c$ nodes, plus a source $s$ and a sink $s'$. In particular, there are $d$ nodes for each colluder, representing their possible bids. For $i \in N_c$ and $j \in [d]$, we let $(i,\bar{b}^c_j)$ be the node representing the bid $\bar{b}^c_j$ for bidder $i$.
%	%
%
%The set of arcs $A$ has cardinality $O(d^2n_c)$. In particular, the source $s$ is connected to nodes $(1,\bar{b}^c_j)$ and nodes $(n,\bar{b}^c_j)$ are connected to the sink $s'$, for all $ j \in [d]$. For every $ i \in N_c \setminus \{1,n\}$ and $ j'\in [d]$, node $(i,\bar{b}^c_{j'})$ is connected to nodes $(i+1,\bar{b}^c_{j})$ with $j \in [d]: j \geq j'$. This implies that in each path the bids are ordered according to the colluders's indexes. This is w.l.o.g. by Lemma \ref{lem_bidorder}. We denote the arc from $(i,\bar{b}^c_{j'})$ to $(i+1,\bar{b}^c_{j})$ with the tuple $(i,\bar{b}^c_{j'},\bar{b}^c_{j})$.
%	%
%
%Each arc $(i,\bar{b}^c_{j'},\bar{b}^c_{j})$ has a weight $w_{i,j',j}$.
%	%
%	For $i \in N_c \setminus \{n\}$ and $j',j \in [d]$, $w_{i,j',j}$ is a fraction of the cumulative utility, once fixed the bids $b_{i'}^c$ with $i'<i$, $b^c_i = \bar{b}^c_{j'}$, and $b^c_{i+1}=\bar{b}^c_j$.
%	%
%	We denote the weights on arcs from nodes $(n,\bar{b}^c_{j'})$ to the sink $s'$ by $w_{n,j',s'}$, while those on arcs from the source $s$ to agent $1$'s nodes are $w_{s,j}=0$, for all $ j \in [d]$. 
%	%

We build the graph as follows (see Figure~\ref{fig:graph}).
\begin{itemize}
	\item The set of vertices $V$ contains $d n_c$ nodes, plus a source $s$ and a sink $s'$. There are $d$ nodes for each colluder, one for each possible bids. For $i \in N_c$ and $j \in [d]$, we let $(i,\bar{b}^c_j)$ be the node representing the bid $\bar{b}^c_j$ for bidder $i$.
	%
	\item The set of arcs $A$ has cardinality $O(d^2n_c)$. The source $s$ is connected to nodes $(1,\bar{b}^c_j)$ and nodes $(n,\bar{b}^c_j)$ to the sink $s'$, for all $ j \in [d]$. For every $ i \in N_c \setminus \{1,n\}$ and $ j'\in [d]$, node $(i,\bar{b}^c_{j'})$ is connected to nodes $(i+1,\bar{b}^c_{j})$ with $j \in [d]: j \geq j'$. This implies that in each path the bids are ordered according to the colluders's indexes. This is w.l.o.g. by Lemma \ref{lem_bidorder}. In the following, we denote the arc from $(i,\bar{b}^c_{j'})$ to $(i+1,\bar{b}^c_{j})$ with the tuple $(i,\bar{b}^c_{j'},\bar{b}^c_{j})$.
	%
	\item Each arc $(i,\bar{b}^c_{j'},\bar{b}^c_{j})$ has a weight $w_{i,j',j}$.
	%
	For $i \in N_c \setminus \{n\}$ and $j',j \in [d]$, $w_{i,j',j}$ is a fraction of the cumulative utility, once fixed the bids $b_{i'}^c$ with $i'<i$, $b^c_i = \bar{b}^c_{j'}$, and $b^c_{i+1}=\bar{b}^c_j$.
	%
	We analogously denote the weights on arcs from nodes $(n,\bar{b}^c_{j'})$ to the sink $s'$ by $w_{n,j',s'}$, while those on arcs from the source $s$ to agent $1$'s nodes are $w_{s,j}=0$, for all $ j \in [d]$. 
	%
\end{itemize}
%
%Figure~\ref{fig:graph} reports a simple example of the graph.


%
A \emph{directed path} $\sigma \in \Sigma$ is a sequence of arcs connecting the source $s$ to the sink $s'$. The \emph{length} $W_\sigma$ of path $\sigma$ is the sum of the weights of the arcs in the path:
\begin{align}
	W_\sigma = \sum_{(i,\bar{b}^c_{j'},\bar{b}^c_{j}) \in \sigma} w_{i,j',j}.
\end{align}
The shortest path problem on the weighted graph is
\begin{align} 
	\min_{\sigma \in \Sigma} - W_\sigma \label{obj_short}.
\end{align}
%
We let $n(b^c_i) \coloneqq \sum_{j=1}^{n_e} \mathbbm{1}_{\{b^e_j > b^c_i\}}$ be the number of external agents with a bid larger than agent $i$'s bid.
%, while $n_i(b^e_j) \coloneqq \sum_{k=1}^{i} \mathbbm{1}_{\{b^c_k \geq b^e_j\}}$ is the number of colluders preceding $i$ (included) with a bid larger than or equal to external bid $b^e_j$.
%

In the GSP mechanism, we define the weight of $(i,\bar{b}^c_{j'},\bar{b}^c_{j})$ as 
%
\begin{align}
w_{i,j',j} = &\lambda_{i+n(b^c_i)} \Big(\hat{y}_i v_i  - \hat{x}\max\Big\{ b^c_{i+1},\max_{b^e_j < b^c_i}{b^e_j}\Big\}\Big),
\end{align}
%
where $b^c_{i} = \bar{b}^c_{j'}$ and $b^c_{i+1} = \bar{b}^c_{j}$.
%
%\textcolor{red}{se soglie = set bid e no weighted utility
%\begin{align}
%	w_{i,j',j} = w_{i,j'} =  \lambda_{i+n(b^c_{i})} \mleft(v_i - b^c_{i}\mright),
%\end{align}}
%
Notice that, under GSP payments, the weight $w_{i,j',j}$ is equal to $u_i^{\w}(b^c)$ when colluder $i$ is assigned to the $(i+n(b^c_i))$-th slot.
%
%Notice that weight $w_{i,j',j}$ is agent $i$'s expected weighted utility under GSP mechanism, which we denote by $u_i^{\w,\GSP}(b)$. 
%
%Colluder $i$ is assigned to the $(i+n(b^c_i))$-th slot and pays $\max\{ b^c_{i+1},\max_{b^e_j < b^c_i}{b^e_j}\}$ scaled by $\hat{x}$. Wieght $w_{i,j',j}$ is composed of agent $i$'s expecetd revenue $r_i(b)=\lambda_{i+n(b^c_{i})} v^c_i$ and payment $\pi^{\GSP}_i(b) = \lambda_{i+n(b^c_{i})} \max\{ b^c_{i+1},\max_{b^e_j < b^c_i}{b^e_j}\}$, respectively scaled by $\hat{y}_i$ and $\hat{x}$.

In the VCG mechanism, we define the weights as follows 
\begin{align}
	&w_{i,j',j} = \hat{y}_i r_{i}(b^c, b^e) - \hat{x} \Big[ g_i(b^c, b^e) + \ell_i(b^c, b^e) \Big], 
\end{align}
where
\begin{align}
	&r_{i}(b) = \lambda_{i+n(b^c_i)} v_i, \\
	& g_i(b) =  (i-1) b^c_i (\lambda_{i + n(b^c_i) - 1} - \lambda_{i + n(b^c_i)}),\\
	&\ell_i(b)=  \sum_{b^e_h \in (b^c_{i+1},b^c_i]} i \, b^e_h (\lambda_{h+i-1} - \lambda_{h + i}),
\end{align}
$b^c_{i} = \bar{b}^c_{j'}$, and $b^c_{i+1} = \bar{b}^c_{j}$. 
% \textcolor{red}{come mai definivamo $n_i(b^e_h)?$ mi sembra sia uguale a $i$}.
%
In the VCG mechanism, $w_{i,j',j}$ has a less intuitive interpretation than for the GSP mechanism.
%
In particular, $w_{i,j',j}$ is composed of a revenue term, which is agent $i$'s expected revenue $r_i(b)=\lambda_{i+n(b^c_{i})} v_i$, weighted by $\hat{y}_i$, and two payment terms, $g_i(b)$ and $\ell_i(b)$, weighted by $\hat{x}$.
%
The latter are two parts of the cumulative payment from the agency to the mechanism, related to the externalities of agents $i' \in N_c$, with $i' <i$, when agents $i$ and $i+1$ bid $b^e_{j'}$ and $b^e_{j}$, respectively.
%expressing the partial expected payments of agents $i'$, with $i' <i$, due to the bid of agents $i$ and $i+1$, \emph{i.e.}, $b^e_{j'}$ and $b^e_{j}$ respectively. 
In particular, the fraction of the expected payment $\pi_{i'}(b)$ related to agent $i'$, with $i'<i$, due to the presence of agent $i$ bidding $b^c_i$, is $b^c_i (\lambda_{i + n(b^c_i) - 1} - \lambda_{i + n(b^c_i)})$. Term $g_i(b)$ is the summation of such payments over all agents $i'$. Moreover, agent $i'$'s fraction of expected payment due to the presence of external agents bidding $b^e_h$ is $b^e_h (\lambda_{h+i-1} - \lambda_{h + i})$. Term $\ell_i(b)$ is the summation of such expected payments due to external agents with bid $b^e_h\in (b^c_{i+1},b^c_i]$.



The following lemma establishes the relation between the length of the paths in the graph and the objective of Problem~\eqref{obj_wup_fix}.
%
\begin{restatable}{lemma}{MapPath}\label{lem_map}
	Consider a path $\sigma \in \Sigma$ composed by the sequence of nodes $\{(1,\bar{b}^c_j), \ldots, (n,\bar{b}^c_{j'})\}$. Then,
	\begin{align} \label{eq_pathbid}
		W_\sigma = \sum_{i \in N_c} \hat{y}_i r_i(b^c, b^e) - \hat{x} \pi_i(b^c, b^e),
	\end{align}
which is the weighted utility in Problem~\eqref{obj_wup_fix} with fixed external bids $b^e$ and bidding strategy $b^c = (\bar{b}^c_j, \ldots, \bar{b}^c_{j'}) \in \bar{B}^c$. Moreover, for each bidding strategy $b^c = (\bar{b}^c_j, \ldots, \bar{b}^c_{j'}) \in \bar{B}^c$ there exists a corresponding path $\sigma \in \Sigma$ composed by the sequence of nodes $\{(1,\bar{b}^c_j), \ldots, (n,\bar{b}^c_{j'})\}$.
\end{restatable}
%
%= &\sum_{i \in N^c}
%\bigg(v_i \lambda_{i+n(b^c_i)} -  (i-1) b^c_i (\lambda_{i + n(b^c_i) - 1} - \lambda_{i + n(b^c_i)})\nonumber\\
%&-\sum_{h \in (j',j]} n(b^e_h) b^e_h (\lambda_{h+n(b^e_h)-1} - \lambda_{h + n(b^e_h)})\bigg)\\
%

The following theorem provides the polynomial-time algorithm solving Problem~\eqref{obj_wup_fix}, which works by simply finding a shortest path of the graph.
%
\begin{restatable}{theorem}{polyweight}\label{th_poly_1}
	There exists a polynomial-time algorithm which solves Problem~\eqref{obj_wup_fix}. 
\end{restatable}

% \textcolor{red}{i weights sui nostri archi possono essere negativi in VCG? SI, vedere come scrivere proof sopra}

Finally, by substituting the quantities involved in Problem~\eqref{obj_wup_fix} with their expectations, thanks to the linearity of the objective we get that:
%
\begin{restatable}{theorem}{PolyExpectation}\label{th_poly}
	There exists a polynomial-time algorithm which solves Problem~\eqref{obj_wup}.
	% in expectation w.r.t. the stochasticity of the profile of external agents'bids. 
\end{restatable}



















==> paper Arxiv 1/contents/transferrableDue.tex <==

\section{Arbitrary Transfers Setting}\label{sec:arbitrary}

In this section, we provide an approximate solution to the media agency problem with arbitrary transfers.
%
In particular, we design a bi-criteria FPTAS that returns solutions providing an arbitrary small loss $\varepsilon > 0$ with respect to the optimal value of the problem, by relaxing the IC constraints by the additive factor $\varepsilon$.
%
As a first step, we show that there always exists a non-randomized solution to Problem~\eqref{lp:problem1}.

\begin{restatable}{lemma}{DetSolution}\label{lem_deterministic}
	In the arbitrary transfers setting, there always exists an optimal non-randomized solution to Problem~\eqref{lp:problem1}.
\end{restatable}

Then, we show how to reduce the problem to a new one working with a finite (discretized) set of bids, in order to apply the results provided in Section~\ref{sec:weighted}.
%
As a first result, given a probability value $p\in [0,1]$ and a minimum discretization step $\eta \in [0,1]$, we show how to split the space of bids $[0,1]$ into a suitably-defined set of intervals using the recursive algorithm whose pseudo-code is provided in Algorithm~\ref{alg}.\footnote{In Algorithm~\ref{alg}, we assume that we can compute some probabilities exactly. It is easy to extend our results---with only a small approximation error---to the case in which the algorithm has access only to samples of the probability distribution over the external bids.}

\begin{algorithm}[!htp] 
	\caption{$\textsc{Rec}((\alpha,\beta],p,\eta)$}\label{alg}
	\textbf{Input:} interval $(\alpha,\beta]\subseteq [0,1]$; probability $p\in [0,1]$; minimum discretization step $\eta \in [0,1]$
	\begin{algorithmic}[1]
		 \IF{$\underset{b^e \sim \gamma^e}{\mathbb{P}} \left\{ \exists j \in N_e: b^e_j \in (\alpha,\beta] \right\}\le p \vee \beta-\alpha \le \eta$} \label{line}
		\RETURN $\{(\alpha,\beta]\}$
	   \ELSE
	   \STATE { $\mathcal{I}_\text{L} \gets \textsc{Rec}\left( \left(\alpha,\frac{\alpha+\beta}{2}\right],p,\eta \right)$}
	   \STATE {$\mathcal{I}_\text{R} \gets \textsc{Rec}\left( \left( \frac{\alpha+\beta}{2}, \beta \right],p,\eta \right)$}
	   \RETURN $\mathcal{I}_{L} \cup \mathcal{I}_\text{R}$
	   \ENDIF
	\end{algorithmic} 
\end{algorithm}


We prove the following:
%
\begin{restatable}{lemma}{REC}\label{lem_REC}
	 Given $p \in [0,1]$ and $\eta \in [0,1]$, $\textsc{Rec}((0,1], p,\eta)$ returns a set $\{(\alpha_j,\beta_j]\}_{j \in [k^*]}$ composed of $k^*\le \frac{2 n_e}{p} \log{ \frac{1}{\eta}}$ intervals such that, for every interval $(\alpha_j,\beta_j]$, it holds either $\mathbb{P}_{b^e \sim \gamma^e} \left\{ \exists i \in N_e: b^e_i \in (\alpha_j,\beta_j] \right\} \le p$ or $\beta_j-\alpha_j\le \eta$.
	 %
	 Moreover, it holds that $\bigcup_{j \in [k^*]} (\alpha_j,\beta_j] =(0,1]$ and the procedure runs in time polynomial in $n_e$, $\frac{1}{p}$, and $\log \frac{1}{\eta}$.
\end{restatable}

Let $I^{p,\eta} \coloneqq \{(\alpha_j,\beta_j]\}_{j \in [k^*]}$ be the set of intervals returned by $\textsc{Rec}((0,1], p,\eta)$.
%
The next step is to show that, for $\eta$ small enough, $\mathbb{P}_{b^e \sim \gamma^e} \left\{ \exists i \in N_e: b^e_i \in (\alpha_j,\beta_j) \right\}\le p$ for every interval $(\alpha_j,\beta_j]$.
%
This holds by definition for each interval $(\alpha_j,\beta_j]$ with $\beta_j-\alpha_j>\eta$.
%
Thus, let us consider the intervals $(\alpha_j,\beta_j]$ such that $\beta_j-\alpha_j\le \eta$.
%
Let $M$ be the maximum number of bits needed to represent the bids $b^e_i$ that are in the support of probability distribution $\gamma^e$.
%
By setting $\eta=2^{-M}$, we have that all the bids $b^e_i$ in the interval $(\alpha_j,\beta_j]$ are equal to $\beta_j$.\footnote{Our algorithm runs in time logarithmic in $\frac{1}{\eta}$ and hence polynomial in the size of the binary representation of bids $b^e$.}
%
Hence, it holds $\mathbb{P}_{b^e \sim \gamma^e} \left\{ \exists i \in N_e: b^e_i \in (\alpha_j,\beta_j) \right\}=0$.


Now, we define the set of discretized bidding strategies $B^{c,p}$ employed in the rest of the paper, as $B^{c,p} \coloneqq \bigcup_{(\alpha,\beta] \in I^{p,\eta}} \bigcup_{i \in N_c}\{\alpha+\tau i\}$ for a small $\tau > 0$ and $\eta=2^{-M}$.\footnote{In the following, we ignore the loss in cumulative expected utility that results from the introduction of $\tau > 0$. Notice that this parameter is only necessary to induce specific tie-breaking rules and our results can be easily extended to consider the loss in utility due to $\tau$. Moreover, $\tau$ can be taken to be exponentially small in the size of the problem instance, and hence negligible.}
%
Next, we show that we can restrict to bid profiles $B^{c,p}$ with a small loss in utility and by relaxing IC constraints.

First, we provide the following auxiliary result.
%
\begin{restatable}{lemma}{DiscretizedBid}\label{lm:discretized}
	Given $p \in [0,1]$, for any bidding strategy $b^c \in B^c$, there exists a discretized bidding strategy $\hat b^c \in B^{c,p}$:
	\begin{itemize}
		\item $ \tilde \pi_i(\hat b^c) \le \tilde \pi_i( b^c)  $ for all $ i \in N_c$; and
		\item $ \tilde r_i(\hat b^c) \ge \tilde r_i( b^c) -p $ for all $  i \in N_c $.
	\end{itemize}
\end{restatable}



Then, by exploiting Lemma~\ref{lm:discretized} we can prove the following Lemma~\ref{lm:arbitrary}.
%
Intuitively, the lemma shows that, given a probability $p\in [0,1]$ and an optimal discretized  bidding strategy $\hat{b}^c \in \argmax_{b^c \in B^{c,p}} \sum_{i \in N_c} \tilde r_i(b^c) - \tilde \pi_i(b^c)$, one can find an approximate solution to Problem~\ref{lp:problem1} in polynomial time.
%
% Formally:
%
\begin{restatable}{lemma}{Arbitrary} \label{lm:arbitrary}
	Given $p\in [0,1]$ and an optimal discretized bidding strategy $\hat b^{c} \in \argmax_{b^c \in B^{c,p}}  \sum_{i \in N_c} \tilde r_i(b^c) - \tilde \pi_i(b^c)$, we can find in polynomial time a $p$-IC and IR solution to Problem~\eqref{lp:problem1} with value at least $OPT-p n_c$, where $OPT$ is the optimal value of Problem~\eqref{lp:problem1}.
\end{restatable}

By Theorem~\ref{th_poly}, for any probability $p \in [0,1]$, it is possible to find an optimal discretized bidding strategy $\hat b^{c} \in \argmax_{b^c \in B^{c,p}  }  \sum_{i \in N_c} \tilde r_i(b^c) - \tilde \pi_i(b^c)$ in time polynomial in the instance size and in $\frac{1}{p}$, since, as it is easy to check, the number of possible discretized bids in $B^{c,p}$ is polynomial in $\frac{1}{p}$.
%
Moreover, by employing Lemma~\ref{lm:arbitrary}, we can use the bidding strategy $\hat b^{c}$ to find an approximated solution to Problem~\eqref{lp:problem1} in polynomial time.
%
Hence, given any $\varepsilon>0$, it is sufficient to choose $p \in [0,1]$ so that $\frac{1}{p} \in \text{poly}(\frac{1}{\varepsilon},n)$ in order to obtain an $\varepsilon$-IC and IR approximate solution to Problem~\ref{lp:problem1}, as stated by the following theorem.
%
\begin{theorem}
	Given $\varepsilon>0$, there exists an algorithm that runs in time polynomial in the instance size and $\frac{1}{\varepsilon}$, which returns an $\varepsilon$-IC and IR solution to Problem~\eqref{lp:problem1} with value at least $OPT-\varepsilon$, where $OPT$ is the optimal value of Problem~\eqref{lp:problem1}.
\end{theorem}



